Universal gauge-invariant cellular automata

Gauge symmetries play a fundamental role in Physics, as they provide a mathematical justification for the fundamental forces. Usually, one starts from a non-interactive theory which governs `matter', and features a global symmetry. One then extends the theory so as make the global symmetry into a local one (a.k.a gauge-invariance). We formalise a discrete counterpart of this process, known as gauge extension, within the Computer Science framework of Cellular Automata (CA). We prove that the CA which admit a relative gauge extension are exactly the globally symmetric ones (a.k.a the colour-blind). We prove that any CA admits a non-relative gauge extension. Both constructions yield universal gauge-invariant CA, but the latter allows for a first example where the gauge extension mediates interactions within the initial CA.

==> Standard_conf.tex <==
\definecolor{gaugeCol}{rgb}{0.40390625,0.6109375,0.09109375}
\definecolor{evolutionCol}{rgb}{0.3,0.3,0.3}
\definecolor{gaugeCol}{rgb}{0.40390625,0.6109375,0.09109375}
\definecolor{evolutionCol}{rgb}{0.3,0.3,0.3}
\definecolor{grayCol}{rgb}{0.6,0.6,0.6}

\newcommand{\stateTikz}[6]{
  \draw[color=#5, #6, very thick](#1- #3 , #2) rectangle (#1 + #3, #2 + #4);
}

\newcommand{\gaugestate}[5]{
  \ifthenelse{#5 > 0}{\def\mycol{gaugeCol}}{\def\mycol{white}};
  \filldraw[fill=\mycol, very thick](#1- #3 , #2) rectangle (#1 + #3, #2 + #4);
}

\newcommand{\stateTikzz}[7]{%(left,
                            % bottom,
                            % width/2,
                            % height,
                            % left side particle ?,
                            % right side particle ?
                            % other parameters)
\ifthenelse{#5 > 0 \AND #6>0}{\def\mycola{white}}{\def\mycola{black}};
\ifthenelse{#5 > 0}{\def\mycolb{black}}{\def\mycolb{white}};
\ifthenelse{#6 > 0}{\def\mycolc{black}}{\def\mycolc{white}};
\filldraw[color=\mycola, fill=\mycolb, #7, thick](#1- #3 , #2) 
    rectangle (#1 , #2 + #4);
\filldraw[color=\mycola, fill=\mycolc, #7, thick](#1, #2)
    rectangle (#1 + #3 , #2 + #4);
}

\newcommand{\stateTikzzz}[6]{%(left,
                            % bottom,
                            % width/2,
                            % height,
                            % left-right particle color
                            % other parameters)
\ifthenelse{#5 = 0}{\def\mycola{black}\def\mycolb{white}\def\mycolc{white}}{};
\ifthenelse{#5 = 1}{\def\mycola{black}\def\mycolb{white}\def\mycolc{black}}{};
\ifthenelse{#5 = 2}{\def\mycola{black}\def\mycolb{black}\def\mycolc{white}}{};
\ifthenelse{#5 = 3}{\def\mycola{white}\def\mycolb{black}\def\mycolc{black}}{};
\ifthenelse{#5 = 4}{\def\mycola{grayCol}\def\mycolb{white}\def\mycolc{grayCol}}{};
\ifthenelse{#5 = 5}{\def\mycola{grayCol}\def\mycolb{grayCol}\def\mycolc{white}}{};
\ifthenelse{#5 = 6}{\def\mycola{white}\def\mycolb{black}\def\mycolc{grayCol}}{};
\ifthenelse{#5 = 7}{\def\mycola{white}\def\mycolb{grayCol}\def\mycolc{black}}{};
\ifthenelse{#5 = 8}{\def\mycola{white}\def\mycolb{grayCol}\def\mycolc{grayCol}}{};
\filldraw[color=\mycola, fill=\mycolb, #6, thick](#1- #3 , #2) 
    rectangle (#1 , #2 + #4);
\filldraw[color=\mycola, fill=\mycolc, #6, thick](#1, #2)
    rectangle (#1 + #3 , #2 + #4);
}

\newcommand{\linefive}[6]{
	\begin{scope}[shift={(0,#1)}]
        \stateTikzzz{0}{0}{1}{1}{#2}{dotted};
        \stateTikzzz{4}{0}{1}{1}{#3}{};
        \stateTikzzz{8}{0}{1}{1}{#4}{};
        \stateTikzzz{12}{0}{1}{1}{#5}{};
        \stateTikzzz{16}{0}{1}{1}{#6}{dotted};
    \end{scope}
}
\newcommand{\gaugefour}[5]{
    \begin{scope}[shift={(0,#1)}]
        \color{gaugeCol}
        \gaugestate{2}{0.1}{0.4}{0.8}{#2};
        \gaugestate{6}{0.1}{0.4}{0.8}{#3};
        \gaugestate{10}{0.1}{0.4}{0.8}{#4};
        \gaugestate{14}{0.1}{0.4}{0.8}{#5};
    \end{scope}
}

\newcommand{\evenline}[2]{
	\begin{scope}[shift={(0,#1)}]
        \stateTikz{0}{0}{1}{1}{#2}{dotted};
        \stateTikz{8}{0}{1}{1}{#2}{};
        \stateTikz{16}{0}{1}{1}{#2}{dotted};
    \end{scope}
}
\newcommand{\evenout}[2]{
	\begin{scope}[shift={(0,#1)}]
        \draw[color=#2] (1,1) -- (3,3)
                        (9,1) -- (11,3)
                        (7,1) -- (5,3)
                        (15,1) -- (13,3);
    \end{scope}
}
\newcommand{\evenouttwo}[2]{
    \begin{scope}[shift={(0,#1)}]
        \draw[color=#2] (1,1) -- (3.9,2) -- (3.9,3)
                        (7,1) -- (4.1,2) -- (4.1,3)
                        (9,1) -- (11.9,2) -- (11.9,3)
                        (15,1) -- (12.1,2) -- (12.1,3);
        \filldraw[color=#2, fill=white] (4,2) circle (0.3);
        \filldraw[color=#2, fill=white] (12,2) circle (0.3);
    \end{scope}
}

\newcommand{\oddline}[2]{
	\begin{scope}[shift={(0,#1)}]
        \stateTikz{4}{0}{1}{1}{#2}{};
        \stateTikz{12}{0}{1}{1}{#2}{};
    \end{scope}
}
\newcommand{\oddout}[2]{
	\begin{scope}[shift={(0,#1)}]
        \draw[color=#2] (1,3) -- (3,1)
                        (9,3) -- (11,1)
                        (7,3) -- (5,1)
                        (15,3) -- (13,1);
    \end{scope}
}

\newcommand{\oddouttwo}[2]{
    \begin{scope}[shift={(0,#1)}]
        \draw[color=#2, dashed] (-.1, 3) -- (-.1,2) -- (-1,1.6)
                                (16.1,3) -- (16.1,2) -- (17,1.6);
        \draw[color=#2] (3,1) -- (0.1,2) -- (0.1,3)
                        (5,1) -- (7.9,2) -- (7.9,3)
                        (11,1) -- (8.1,2) -- (8.1,3)
                        (13,1) -- (15.9,2) -- (15.9,3);

        \filldraw[color=#2, fill=white] (0,2) circle (0.3);
        \filldraw[color=#2, fill=white] (8,2) circle (0.3);
        \filldraw[color=#2, fill=white] (16,2) circle (0.3);
    \end{scope}
}

\newcommand{\gauge}[1]{
    \begin{scope}[shift={(0,#1)}]
        \foreach \i in {2,6,...,14}{
            \stateTikz{\i}{0.1}{0.4}{0.8}{gaugeCol}{};
        }
    \end{scope}
}
\newcommand{\gaugeout}[1]{
    \begin{scope}[shift={(0,#1)}]
        \foreach \i in {2,6,...,14}{
            \draw[color=gaugeCol] (\i,0.9) -- (\i, 3.1);
        }
    \end{scope}
}

\newcommand{\evolution}[1]{
    \begin{scope}[shift={(0,#1)}]
        \foreach \i in {2,6,...,14}{
            \filldraw[color=evolutionCol, fill=white] (\i,2) circle (0.3);
        }
    \end{scope}
}

\newcommand{\grid}[2]{
    \begin{scope}[shift={(#1,#2)}]
        %axis
        \draw[->, very thick] (-1.5,-0.5) -- coordinate (x axis mid) (17.5,-0.5);
        \draw[->, very thick] (-1.5,-0.5) -- coordinate (y axis mid) (-1.5,7.5);
        %ticks
        \foreach \x in {0,4,...,16}
            \draw[very thick] (\x,-0.4) -- (\x,-0.7);
        \foreach \y in {0.5,3.5,...,6.5}
            \draw[very thick] (-1.7,\y) -- (-1.4,\y); 
        %labels      
        \node at (18,-0.5) {\Huge $x$};
        \node at (-1.5,8) {\Huge $t$};
    \end{scope}
}


\newcommand{\gridgauge}[2]{
    \begin{scope}[shift={(#1,#2)}]
        %axis
        \draw[->, very thick] (-1.5,-0.5) -- coordinate (x axis mid) (17.5,-0.5);
        \draw[->, very thick] (-1.5,-0.5) -- coordinate (y axis mid) (-1.5,7.5);
        %ticks
        \foreach \x in {0,4,...,16}
            \draw[very thick] (\x,-0.4) -- (\x,-0.7);
        \foreach \x in {2,6,...,14}
            \draw[very thick] (\x,-0.5) -- (\x,-0.6);
        \foreach \y in {0.5,3.5,...,6.5}
            \draw[very thick] (-1.7,\y) -- (-1.4,\y); 
        %labels      
        \node at (18,-0.5) {\Huge $x$};
        \node at (-1.5,8) {\Huge $y$};
    \end{scope}
}


\definecolor{gaugeCol}{rgb}{0.40390625,0.6109375,0.09109375}
\definecolor{evolutionCol}{rgb}{0.3,0.3,0.3}

\begin{tikzpicture}


%%%%% BLACK GRID %%%%%
\evenline{0}{black};
\oddline{3}{black};
\evenline{6}{black};



\oddline{0}{black}
\evenline{3}{black}
\oddline{6}{black}




%%%%% Gauge (base) %%%%%
\gauge{0}
\gauge{3}
\gauge{6}

%%%%% Gauge (ligne 1) %%%%%

\draw[color=gaugeCol,dashed,thick](-0.40,1.5) rectangle (0.40,2.3);
\draw[color=gaugeCol,thick](1.6,1.5) rectangle (2.4,2.3);
\draw[color=gaugeCol,thick](3.6,1.5) rectangle (4.4,2.3);
\draw[color=gaugeCol,thick](5.6,1.5) rectangle (6.4,2.3);
\draw[color=gaugeCol,thick](7.6,1.5) rectangle (8.4,2.3);
\draw[color=gaugeCol,thick](9.6,1.5) rectangle (10.4,2.3);
\draw[color=gaugeCol,thick](11.6,1.5) rectangle (12.4,2.3);
\draw[color=gaugeCol,thick](13.6,1.5) rectangle (14.4,2.3);
\draw[color=gaugeCol,dashed,thick](15.6,1.5) rectangle (16.4,2.3);

%%%%% Gauge (ligne 2) %%%%%

\draw[color=gaugeCol,dashed,thick](-0.40,4.6) rectangle (0.40,5.4);
\draw[color=gaugeCol,thick](1.6,4.6) rectangle (2.4,5.4);
\draw[color=gaugeCol,thick](3.6,4.6) rectangle (4.4,5.4);
\draw[color=gaugeCol,thick](5.6,4.6) rectangle (6.4,5.4);
\draw[color=gaugeCol,thick](7.6,4.6) rectangle (8.4,5.4);
\draw[color=gaugeCol,thick](9.6,4.6) rectangle (10.4,5.4);
\draw[color=gaugeCol,thick](11.6,4.6) rectangle (12.4,5.4);
\draw[color=gaugeCol,thick](13.6,4.6) rectangle (14.4,5.4);
\draw[color=gaugeCol,dashed,thick](15.6,4.6) rectangle (16.4,5.4);



%%%%% Grid %%%%%
\gridgauge{0}{0}

\end{tikzpicture}
